Degrees of extensionality in the theory of B\"ohm trees and Sall\'e's conjecture

The main observational equivalences of the untyped lambda-calculus have been characterized in terms of extensional equalities between B\"ohm trees. It is well known that the lambda-theory H*, arising by taking as observables the head normal forms, equates two lambda-terms whenever their B\"ohm trees are equal up to countably many possibly infinite eta-expansions. Similarly, two lambda-terms are equal in Morris's original observational theory H+, generated by considering as observable the beta-normal forms, whenever their B\"ohm trees are equal up to countably many finite eta-expansions. The lambda-calculus also possesses a strong notion of extensionality called "the omega-rule", which has been the subject of many investigations. It is a longstanding open problem whether the equivalence B-omega obtained by closing the theory of B\"ohm trees under the omega-rule is strictly included in H+, as conjectured by Sall\'e in the seventies. In this paper we demonstrate that the two aforementioned theories actually coincide, thus disproving Sall\'e's conjecture. The proof technique we develop for proving the latter inclusion is general enough to provide as a byproduct a new characterization, based on bounded eta-expansions, of the least extensional equality between B\"ohm trees. Together, these results provide a taxonomy of the different degrees of extensionality in the theory of B\"ohm trees.

==> include/fig_etamax.tex <==
% !TEX root = ../IntrigilaMP18.tex
{\small
\begin{figure*}[t!]
\[
~~\etamax \code{M} \code{N} s
= 
\begin{cases}
	\lam \fresh{x_1}\dots \fresh{x_n}. \bP_q s (\fresh{x_j} (\Upsilon_1 \fresh{x_1}\cdots\fresh{x_n}) \cdots (\Upsilon_k \fresh{x_1}\cdots\fresh{x_n}))
&
\text{if } M\le_h N,\textrm{ with }\\
 \text{where}\left[
\!\! \begin{array}{l}
	q =\iota(\num{\NF[\beta](\lam \fresh{y} z_1 \dots z_m.\fresh{y} Q_1 \cdots Q_m)})\\
	\Upsilon_i := \etamax \code{\lam x_1\dots x_n.M_i} \code{\lam x_1\dots x_n.N_i} s
  \end{array}\right.
&
\begin{array}{l}
M \msto[h] \lam  x_1\dots x_n. x_j M_1 \cdots M_k\textrm{ and }\\
N\msto[h]  \lam x_1\dots x_n  z_1\dots z_m. x_j N_1 \cdots N_k Q_1 \cdots Q_m;\\
\end{array}
\\
\etamax \code{N} \code{M} s&\text{if } N <_h M;\\[2pt]
\Omega&\text{otherwise.}
\end{cases}
\]
\caption{The \lam-term $\etamax\in\Lamo$ satisfies in $\cH$ the recursive equation above (where the underlined variables are fresh). }\label{fig:etamax}
\end{figure*}
}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../IntrigilaMP18.tex"
%%% End:


==> include/fig_kite.tex <==
% !TEX root = ../IntrigilaMP18.tex
\begin{figure}[t!]

\caption{, where $\cT$ is above $\cT'$ if $\cT\subsetneq \cT'$.}\label{fig:kite}
\end{figure}  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../IntrigilaMP18.tex"
%%% End:

